Correlation visualization under missing values: a comparison between imputation and direct parameter estimation methods

Correlation matrix visualization is essential for understanding the relationships between variables in a dataset, but missing data can pose a significant challenge in estimating correlation coefficients. In this paper, we compare the effects of various missing data methods on the correlation plot, focusing on two common missing patterns: random and monotone. We aim to provide practical strategies and recommendations for researchers and practitioners in creating and analyzing the correlation plot. Our experimental results suggest that while imputation is commonly used for missing data, using imputed data for plotting the correlation matrix may lead to a significantly misleading inference of the relation between the features. We recommend using DPER, a direct parameter estimation approach, for plotting the correlation matrix based on its performance in the experiments.

==> Sections/introduction_and_related_work.tex <==
% In this paper, we analyze the global effect of using different covariance matrix estimation approaches to correlation plot, a common visualization technique. These include DPER* and imputing by missForest/MICE/.... (you can select the ones like in the DIMV paper) and then estimate covariance matrix from imputed data.

% For this, we mainly show the plots, to see how the resulted plots are visually significantly different 

% https://stackoverflow.com/questions/29432629/plot-correlation-matrix-using-pandas

% https://seaborn.pydata.org/generated/seaborn.heatmap.html

% In statistics, the correlation matrix is a commonly used tool to understand the relationship between different variables in a dataset. Visualization of the correlation matrix is essential in understanding the relationship between variables. However, correlation matrix estimation becomes challenging when the dataset has missing values. The presence of missing values in the data can bias the correlation estimates and lead to incorrect conclusions. In recent years, there has been a growing interest in developing methods to handle missing data in correlation analysis. In this paper, we survey various ways of visualizing the correlation matrix when missing values exist in the dataset with different missing patterns. Our goal is to provide an overview of available methods for visualizing correlations under missing values. To achieve this, we will compare and evaluate different techniques, highlighting their advantages and disadvantages.  


% The correlation of data plays a vital role in statical learning and machine learning. Visualizing the correlation between features helps identify the patterns and relationships between variables. The correlation is also a proxy of the covariance matrix, which is critical in many machine-learning models. There are many reasons that correlation/covariance estimation is essential in machine learning. In feature selection, correlations help identify collinearity and remove duplicative features in the dataset. The covariance matrix is used in Principal Component Analysis to identify the essential elements in a dataset, which help us reduce the dimensionality of the dataset and build more efficient models. Some regularization techniques, such as Ridge and Lasso regression, also use covariance to add a penalty term to the model's loss function proportional to the covariance between the model parameter to prevent the model from overfitting.

% Correlation visualization is an initial yet important step in modern statistical data analysis. Multiple graphical techniques can help figure out associations of variables, such as scatter plots, heat maps, correlation matrices, networks graph, etc. One of the most popular is using matrix visualization with heat maps to quickly get information about the magnitude and direction of the relationship. Correlation matrix heat maps help to gain insight via exploratory data analysis. The visualization also can aid in model interpretability for the results of a deep learning model by identifying which features are most strongly associated with the predicted outcomes.

% write more about missing data tyoe here 


% Missing data is an inevitable issue in data collection, which introduces bias into our analysis and prediction process. In this scenario, the estimation of correlation/covariance estimation requires a missing data handling technique. However, the correlation visualization technique become harder when data is missing. A simple approach to handling the missing data is using case completion, which excludes all cases in which either one or both of the correlated values are missing. The more advance approach is to use different single and multiple imputation techniques, which allows us to do statistical estimation and inference when missing data exists. Or another method is to directly estimate the correlation or covariance matrix, in which the data does not need to be imputed inadvance. In this paper, we analyze the effect of different correlation matrix estimation approaches and visualize them with the standard technique - the correlation plot.


% Our contributions are as follows:
% \begin{itemize} 
%     \item We examine the effect of different methods to graphically estimate the correlation matrix (including methods with and without imputation) using the correlation matrix heat maps.
%     \item We compare the result of the correlation estimation using RMSE (root mean square error) as a metric for on different datasets and different missing patterns including randomly missing pattern and monotone missing pattern. 
% \end{itemize} 


%introduce cm & missing data trong cm
% Group Solution :
    % imputation: mising data -> visualize : related.
    % directly estimate : DPER (paper)
% Contribution
    



Correlation visualization is an initial yet important step in modern statistical data analysis and building machine learning models. This is because a correlation matrix is a powerful statistical tool to summarise data sets, reveal relationships between variables, and identify patterns in the given data set. However, missing values can make correlation matrix estimation challenging, leading to biased estimates and incorrect conclusions. Recent research focuses on developing methods to handle missing data in correlation analysis. 

% . This paper surveys visualization techniques for correlation matrices with missing values to compare and evaluate different methods.  %and highlight their pros and cons.  

Missing data is a common issue in data collection that can introduce bias
into analysis and prediction. Handling missing data is crucial for estimating the correlation/covariance matrix. Case completion, which excludes cases with missing data, is a simple approach. More advanced methods include single and multiple imputation techniques or direct estimation of the correlation/covariance matrix. This paper examines different approaches for estimating correlation matrices and visualizes them using a standard correlation plot. 


%Missing data is a common issue in statistical analysis, including the estimation of correlation matrices.
%\textbf{(1st approach)}  
The first approach we mention in this paper is imputing missing values, then computing the correlation matrix.  Various methods have been proposed to handle missing data and can be categorized based on the underlying statistical, machine learning, or deep learning methods.
Firstly, \textbf{statistical methods} involve some assumptions about the distribution of the data to estimate the plausible value for the missing positions. Some popular methods in this group include mean imputation, regression, and Expectation maximization. Statistical methods are usually fast and easy to implement, the results are interpretable and provide the uncertainty for the estimation, which is generally presented via the confidence interval. 
%Mean imputation is a widely used and simple method for handling missing data, but it can introduce bias when dealing with a large amount of missing data. 
%The EM algorithm iteratively estimates parameters in statistical models with missing data, alternating between the E-step and the M-step until convergence. 
%One drawback of the EM algorithm is that it can get stuck in local maxima and may not always converge to the global maximum.
% Regression based
%Regression-based models are also common approaches. They are applied in an iterative manner, which is known under the names regression switching, chain equations (MICE \cite{buuren2010mice}) or sequential regression,  are commonly used to handle missing data, but they can be slow with large datasets, despite being flexible and relatively easy to implement. 
Secondly, \textbf{machine learning} techniques train on the available data to learn patterns and relationships and then are used to predict the missing values. There are many typical approaches, including clustering-based methods (KNN Imputation \cite{KNNImputation2001TrevorHastie}),tree-based models (MissForest \cite{stekhoven2012missforest}), matrix completion (\cite{candes2009exact}), methods based on Bayesian Networks (\cite{hruschka2007bayesian}, \cite{audigier2016multiple})  and some other techniques use extreme learning machine (\cite{sovilj2016extreme}). They have their own advantages and disadvantages, and in general, the common drawback is that they can be computationally expensive for large data sets.
% % moving fuzziness method to clustering. 
% Among the classical methods that apply machine learning techniques, the K-Nearest Neighbor (KNNImputation) \cite{KNNImputation2001TrevorHastie} is one of the most widely used ones. The basic idea of KNN-based algorithm is to use a distance function to acquire k samples that are most similar to the samples of interest, then use these k samples to calculate an estimation for the missing values. However, the classical K-Nearest Neighbor (KNN) can ignore the statistical correlation between the different attributes of a sample. An extension of KNN imputation is the Fuzzy K-Means Clustering methods \cite{temp} , where a sample belongs partially to multiple clusters. \cite{temp} utilize a fuzzy c-means clustering hybrid approach in which the fuzzy clustering parameters, cluster size and weighting factor are optimized.  \textcolor{}
% Clustering-based imputation is another branch of machine learning imputation technique apply an unsupervised learning technique to group a set of similar objects into the same cluster. Then estimation for missing values is based on values between incomplete data and the identified cluster centroids. K-means Clustering Imputation (KMI) [cite] is a simple and popular clustering-based technique in which data is divided into two parts: complete data and incomplete. Clusters are computed based on complete data, and missing samples are assigned to a group. Several methods are developed based in this technique. To find an imputation value, a nearest neighbor algorithm can be chosen. KNN consider several nearest neighbor are considered for an (weighted) average. KEMI and kEMI+ (2019) [cite] also use the KNN algorithm for pre-imputation and then use Expectation–Maximization algorithm for posterior imputation.  
 %Among the classical methods that apply machine learning techniques, the K-Nearest Neighbor (KNNImputation) \cite{KNNImputation2001TrevorHastie} is one of the most widely used ones. Other clustering-based imputation methods group similar objects into clusters and estimate missing values based on identified cluster centroids, such as K-means Clustering Imputation (KMI). An extension of KNNImputation is Fuzzy K-Means Clustering methods [cite], which allows a sample to belong partially to multiple clusters. Fuzzy K-Means Clustering utilizes a fuzzy c-means clustering hybrid approach, optimizing the fuzzy clustering parameters, cluster size, and weighting factor. However, these techniques may ignore the statistical correlation between attributes.
 % Tree-based Another common approaches are tree-based models, which can handle missing values in mixed-type data set and they are flexible enough to fit interactions, nonlinear relations and complex distributions without parametric assumptions or data transformations. However, it can be computationally costly for large dataset. The candidate of this group that using in the experiment part is MissForest \cite{stekhoven2012missforest}.  
%Matrix completion is a method for recovering the missing entries of a partially observed matrix. With very high probability, most low-rank matrices can be perfectly recovered from a sampling of their entries by solving a simple convex optimization program \cite{candes2009exact}. The defect of matrix completion methods is that they can be costly as matrix sizes and ranks increase.
%Imputation methods based on Bayesian Networks, such as \cite{garcia2005naive} and \cite{hruschka2007bayesian}, preserve statistical relationships between variables, while \cite{audigier2016multiple} conducts multiple imputations using a Bayesian treatment of the principal component analysis model.
% % Extreme methods Some other techniques use extreme learning machine, which is feedforward neural networks, but instead of using gradient descent to compute weights, it uses the Moore-Penrose generalized inverse, for example AAELM \cite{sovilj2016extreme}, but the work of estimate the inverse is costly. 
Finally, \textbf{Deep Learning} is an emerging trend for handling missing data, where different architectures such as denoising autoencoders, generative models, and graph neural networks are employed. Variational Autoencoder (\cite{Pierre2019Miwae}, \cite{MarkCollier2020vaes}), and Generative adversarial networks (\cite{yoon2018gain}) are widely used.
%Variational Auto Encoder variants use latent variable probabilistic models to tackle missing data, including techniques such as \cite{Pierre2019Miwae} and \cite{MarkCollier2020vaes}. Generative adversarial networks are also used, particularly for image data, such as GAIN \cite{yoon2018gain}. 
These methods have achieved high accuracy, but they require significant computational resources and are best suited for data-rich cases. 



% Imputation models that leverage the advantages of using Bayesian Networks to preserve statistical relationships between variables. These algorithms try to fill missing value by replacing the attribute information according to the probability estimate like \cite{garcia2005naive}.Another method construct the Bayesian Network that represents the data attributes, and introduce searching algorithms on that graph \cite{hruschka2007bayesian}. Or multiple imputations were conducted based on a Bayesian treatment of the principal component analysis model \cite{audigier2016multiple}
 


% % \textcolor{red}{candidate of this group is KNN, mention some advantage and disadvantage of this group (computational cost for, check why it is costly)}

% Other the family of clustering based method is to applies fuzzy clustering to make educated guess base on the groups, some method in this family are \cite{razavi2016imputation}, \cite{rahman2016missing}, \cite{nikfalazar2020missing}. An extension of KNNImputation is the Fuzzy K-Means Clustering methods, where a sample belongs partially to multiple clusters. [ ] utilize a fuzzy c-means clustering hybrid approach in which the fuzzy clustering parameters, cluster size and weighting factor are optimized. 

% % \textcolor{red}{candidate of this group is Gain / VAE, mention some advantage and disadvantage of this group (require large dataset, GINN can be costly)} 


% % Extreme methods 

% Some other techniques use extreme learning machine, which is feedforward neural networks, but instead of using gradient descent to compute weights, it uses the Moore-Penrose generalized inverse, for example AAELM \cite{sovilj2016extreme}, but the work of estimate the inverse is costly. 


% % Deep learning method
% Another emerging trend is using deep learning to handle missing data by employing different architectures, such as denoising autoencoders \cite{gondara2017multiple, marivate2007autoencoder}, generative models, and graph neural networks. Variational Auto Encoder variants as a generative method apply the latent variable generative model in different treatment tackles missing data by using latent variable probabilistic models, including techniques such as \cite{Pierre2019Miwae} \cite{MarkCollier2020vaes}. Other prominent generative frameworks used in imputations are the Generative adversarial networks family, especially for images data, namely GAIN \cite{yoon2018gain} 
% %, (missGAN), (VIGAN), and (CollaGAN). 
% Graph-based framework tackles the missing data problem using a graph representation such as GRAPE \cite{grape2020graph} or GINN \cite{Indro2020ginn}. The deep learning methods have yielded very high accuracy; however, they require high computational costs and just befitting for cases when large amounts of data are available.  
% % Fuzzy Method 

%\textbf{(draw back of imputation before Correlation plot)} 
The above approach has some limitations as follows: first, the algorithms run slowly, especially for large datasets, second, some of them do not preserve the correlation of features in the process filling values, thereby leading to deviations.

To overcome these limitations, we consider the second approach: correlation matrix can also be directly estimated even though the data is missing by using the DPER algorithm \cite{NGUYEN2022108082}. Under some mild assumptions, this algorithm directly calculates the Maximum Likelihood Estimators (MLEs) for the mean and covariance matrix of one-class/multiple-class randomly missing data, whether the data set is small or large. This method does not require many iterations through the data, promising a faster estimation speed. 

 Our contributions are as follows: First, we examine the effect of different methods to graphically estimate the correlation matrix (including methods with and without imputation) using the correlation matrix heat maps. Second, we compare the result of the correlation estimation using RMSE as a metric for different datasets and different missing patterns, including randomly missing patterns and monotone missing patterns. 


%\textbf{The remaining part of this paper is organized as follows.} 
The remaining part of this paper is organized as follows. Section \ref{sec-methods} presents the algorithms concretized from the two approaches introduced and they are under compared in this paper. Next, in section \ref{sec-experiments}, we detail the process of running the experiments and the results for comparing those algorithms. Finally, we draw conclusions and present future development directions to better solve the problem of the correlation matrix under missing values.
